Faster Parallel Exact Density Peaks Clustering

Clustering multidimensional points is a fundamental data mining task, with applications in many fields, such as astronomy, neuroscience, bioinformatics, and computer vision. The goal of clustering algorithms is to group similar objects together. Density-based clustering is a clustering approach that defines clusters as dense regions of points. It has the advantage of being able to detect clusters of arbitrary shapes, rendering it useful in many applications. In this paper, we propose fast parallel algorithms for Density Peaks Clustering (DPC), a popular version of density-based clustering. Existing exact DPC algorithms suffer from low parallelism both in theory and in practice, which limits their application to large-scale data sets. Our most performant algorithm, which is based on priority search kd-trees, achieves $O(\log n\log\log n)$ span (parallel time complexity) for a data set of $n$ points. Our algorithm is also work-efficient, achieving a work complexity matching the best existing sequential exact DPC algorithm. In addition, we present another DPC algorithm based on a Fenwick tree that makes fewer assumptions for its average-case complexity to hold. We provide optimized implementations of our algorithms and evaluate their performance via extensive experiments. On a 30-core machine with two-way hyperthreading, we find that our best algorithm achieves a 10.8--13169x speedup over the previous best parallel exact DPC algorithm. Compared to the state-of-the-art parallel approximate DPC algorithm, our best algorithm achieves a 1.5--4206x speedup, while being exact.

==> baseline.tex <==
\subsection{\citet{Amagata21}'s Algorithm}\label{sec:baseline-amagata}
\shangdi{maybe write a little less here, and write some more details about how DPC is computed in section 2}

\michael{brief descriptions of other algorithms}

\begin{enumerate}
    \item \emph{Density computation:} \citet{Amagata21}'s algorithm constructs a \kdt $T$ from all points. It then computes the density for every point $X_i$ in parallel by $\rho(X_i)\leftarrow T.$\algname{query-range}$(X_i,d_\text{cut})$. 
    \item \emph{Dependent point finding:} 
    \citet{Amagata21}'s algorithm uses a dynamic \kdt $T'$ to find each point's dependent point. It first sorts all points by descending order of density and then sequentially iterate through the sorted points. Point $X_i$'s dependent point is found by $\lambda(X_i)\leftarrow T'.$\algname{query-nn}$(X_i)$. Then, $X_i$ is inserted into dynamic \kdt $T'$.
    \shangdi{discuss visiting all points in range query}
    \citet{Amagata21}, we go down the \kdt, visiting the points in all leaf cells that intersect with $R$.
    \item \emph{Single linkage clustering:} 
    To solve single linkage clustering, \citet{Amagata21}'s algorithm simply performs a depth first search starting from each cluster center. 
\end{enumerate}

The primary computational bottleneck both theoretically and experimentally is the dependent point finding step; this is true especially in low dimensional datasets. Its sequential for loop incurs a high span complexity. Moreover, the dynamic \kdt point insertions could unbalance the \kdt, which does not have trivial re-balancing strategies \cite{Bentley75}. The unbalanced \kdt's height is not bounded by $\BigO{\log(n)}$, causing its $k$-nearest neighbor search work complexity and span complexity to explode from an expected complexity of $\BigO{\log(n)}$ to $\BigO{n}$. As a result, the overall dependent point finding routine has a work and span complexity of $\BigO{n^2}$. The primary focus of our work is proposing faster algorithms to solve the dependent point finding task. 















 













 

 






==> density-comp.tex <==
\section{Improving Density Computation}\label{sec:density-comp}

In this section, we present a simple technique to optimize the density computation operation \algname{query-range}$(X_\text{center}, r)$. Let $S$ denote the spherical region with radius $r$ and centered at $X_\text{center}$ that the query operation intends to inspect. In a standard \algname{query-range} operation used by \citet{Amagata21}, we go down the kd-tree, visiting the points in all leaf cells that intersect with $S$. We note that since we only seek to count the number of points in $S$, we do not have to visit every point. If a cell corresponding to a subtree is contained inside $S$ completely, then we can simply add the number of points inside that cell to the count and prune the subtree from the rest of the traversal. It is possible to check whether a hyper-rectangular region $R$ in coordinate space is contained inside a sphere $S$ by finding a point $X_\text{far}$ \shangdi{This X far is not neccesarrily one of the points in the dataset? I think using X might be confusing, since X is used for points in the dataset} inside $R$ that is farthest from the center of $S$ and checking if $X_\text{far}\in S$. Let $X_\text{min}$ represent the vertex of $R$ with minimal coordinate values in all dimensions and let $X_\text{max}$ represent the vertex with maximal coordinate values. Dimension $i$ of the farthest point, $X^i_\text{far}$, can be found by:

 \begin{algorithmic}[0]
  \If{$X^i_\text{center} < (X^i_\text{min} + X^i_\text{max})/2$} 
    \State $X_\text{far}^i \leftarrow X^i_\text{max}$ 
  \Else
    \State $X_\text{far}^i \leftarrow X^i_\text{min}$ 
  \EndIf

 \end{algorithmic}


\myparagraph{Analysis}

Let $R_S$ represent the smallest hypercube that contains the query region $S$. The runtime of performing range query on $S$ can be bounded by the runtime of performing range query on $R_S$ \cite{Lee77}. \citet{Lee77} proved that the number of cells that intersect with $R_S$ in the kd-tree can be bounded by $\BigO{n^{1-\frac{1}{d}}}$. With the pruning trick we use, all the cells contained inside $R_S$ that our algorithm visits must have parents that are not contained inside $R_S$. Therefore, with this trick, the range counting complexity of \algname{query-range} can be reduced from $\BigO{n^{1-\frac{1}{d}} + \text{size}(S)}$ to $\BigO{n^{1-\frac{1}{d}}}$. 

\shangdi{I think we can merge this section with section 3.4. This is something different from Amagata's implementation, but it's not entirely new, I think some previous work have done this. We can just describe it as an implementation improvement.}


==> priority-kd-tree-theory.tex <==
\section{Priority Search Kd-Tree}\label{sec:priority-search-kd-tree}
We now describe the priority search kd-tree data structure in greater detail. Intuitively, it is a generalization of the 1 dimensional priority search tree data structure to higher dimensions. Each point stored in a priority search kd-tree not only has a $d$ dimensional coordinate value but also a priority value $\gamma$. Each node of the priority search kd-tree corresponds to a set of points and a partition of space---called a cell. At each node, we store the point with the highest $\gamma$ value amongst all points in the point set; this $\gamma$ value is referred to as the $\gamma$ value of the node. The rest of points are split evenly between the children of the node along a hyperplane perpendicular to the longest side of the cell of that node. 

It should be noted that if instead of storing a point with the highest $\gamma$ value at each node, we only store the highest $\gamma$ value, then we arrive at a max kd-tree \cite{Gro07}. \shangdi{do you mean that in max kd-tree, the point with the max gamma value is stored in the left or right subtree, but in the priority search kd-tree, it is stored in the node itself?} We show that both \shangdi{for "both", do you mean the priority search tree and the normal kd-tree?} structures have equivalent expected $k$ nearest neighbor query complexity. However, a priority search kd-tree has a stricter range query complexity bound than a max kd-tree, as shown in Appendix \ref{app:proof-priority-kd-tree-range-query}. \shangdi{missing reference}

Let $T$ denote a priority search kd-tree. Given a query cutoff $\gamma_q$, we let $T_q$ be the subset of $T$ consisting of only nodes with $\gamma$ value $> \gamma_q$. Then, $T_q$ is necessarily a connected tree due to the structural property of a priority search kd-tree. Thus, given a specific query cutoff $\gamma_q$, we can consider a priority search kd-tree to be equivalent to an incomplete kd-tree by letting $T_q$ be the active portion of the tree and the rest of the nodes be the inactive portion. The same argument can be made for a max kd-tree. Therefore, given a specific query cutoff, a max kd-tree can also be considered equivalent to an incomplete kd-tree. Therefore, both structures share the $k$ nearest neighbor query complexity result of an incomplete kd-tree, as shown in Section \ref{sec:complexity}. 

\subsection{Priority Range Query with Priority Search Kd-Tree}

Let $R_q$ denote an axis-parallel rectangular region \shangdi{the proof here is for a rectagular region, but our algorithm uses a query for spherical region} in $d$ dimensional space and $\gamma_q$ denote a threshold value. A priority search kd-tree can be used to answer priority range queries of the form: find all points $X_i\in M$ such that $X_i\in R_q$ and $\gamma_i > \gamma_q$. In the query operation, we traverse down the priority search kd-tree, pruning subtrees with cells that do not intersect $R_q$ and subtrees with $\gamma$ values $\le \gamma_q$.  

\subsubsection{Priority Range Query Complexity Proof}
The time complexity of a priority range query can be bounded by $\BigO{n^{1-\frac{1}{d}} + |Q|}$, where $Q$ is the set of points that satisfy the query conditions. We prove this result by bounding the number of cells in the priority search kd-tree that the query algorithm visits. Note that each cell the kd-tree visits must have a $\gamma$ value greater than $\gamma_q$. We consider two types of such cells.

\myparagraph{The cell is not contained in $R_q$ and only intersects $R_q$}

It is well known that number of such cells in a kd-tree structure is bounded by $\BigO{n^{1-\frac{1}{d}}}$ \cite{CLRS}. 

\myparagraph{The cell is contained within $R_q$}

Each cell $R_i\subseteq R_q$ and $\gamma_i>\gamma_q$ must contain a unique point satisfying the priority range query condition. There are a total of $|Q|$ such points. Therefore, $R_q$ can only enclose $\le |Q|$ cells. 

Thus, we know that the axis-parallel range query runtime for a priority search kd-tree is $\BigO{n^{1-\frac{1}{d}}+|Q|}$. Note that this proof cannot apply to a max kd-tree because the condition that each cell corresponds to one unique point in $Q$ does not hold.


\subsection{$K$ Nearest Neighbor Query with Priority Search Kd-Tree}\label{sec:priority-search-kd-tree:knn}

The objective of a $k$ nearest neighbor search in a priority search kd-tree is to find the $k$ nearest neighbors $X_1, X_2, \cdots, X_k$ of a point $X_q$ such that $\gamma_i > \gamma_q$ for all $i\in[1,k]$. This can be achieved using a similar procedure as the $k$ nearest neighbor search for a normal kd-tree. First, traverse down the tree to find the smallest cell that contains $X_q$ and has a $\gamma$ value $> \gamma_q$. Then, we backtrack up the priority search kd-tree, visiting neighboring sibling subtrees with $\gamma$ values  $>\gamma_q$. If we let $X_q$'s distance to the current $k^\text{th}$ nearest neighbor candidate be denoted by $L^k$, then we can prune the search of any subtree whose cell is at least $L^k$ away from $X_q$. Again, this is effectively the same as performing a $k$ nearest neighbor search on an incomplete kd-tree $T$ with $T_q$ being its active parts. It should also be noted that if we let the $\lambda_i$ value of a point $X_i$ be its density value, then the nearest neighbor problem on a priority search kd-tree is equivalent to the dependent point finding problem. The $k$ nearest neighbor query complexity of a priority search kd-tree is bounded by the query complexity on an incomplete kd-tree. We show in Section \ref{sec:complexity} that the query complexity is $\BigO{\log(n)}$ in expectation. The worst-case complexity is $\BigO{n}$. 






==> single-linkage-cluster.tex <==
\section{Improving Single Linkage Clustering}

The depth first search based single linkage clustering used by \citet{Amagata21} incurs a formidable span complexity of $\BigO{n}$. To improve this span complexity down to $\BigO{\log(n)}$, we opt to use a lock-free parallel union-find data structure \cite{Jayanti21}. Our approach is inspired by \citet{Wang20}'s success in using a parallel union-find data structure to parallelize the DBSCAN algorithm. The procedure is simple and is shown in Algorithm \ref{alg:single-linkage-cluster}. 

\begin{algorithm}[H]
 \footnotesize
\caption{Single linkage clustering with parallel union-find}
 \begin{algorithmic}[1]

 \Procedure{single-linkage-cluster}{$M$, $\lambda$, $\delta$, $\delta_\text{min}$} 
 \State initialize $F$ to be an empty parallel union-find data structure \label{alg:single-linkage-cluster:init}
 \ParFor{all $X_i$ in $M$}
    \If{$\delta(X_i) < \delta_\text{min}$} \Comment{check if $X_i$'s dependent distance is $<$ threshold}
        \State $F.$\algname{unionize}$(X_i, \lambda(X_i))$ \Comment{unionize $X_i$ with $\lambda(X_i)$} \label{alg:priority:unionize}
    \EndIf
 \EndParFor
 \State \Return $F.\text{cluster-labels}$
 
 \EndProcedure
 
 \end{algorithmic}
 \label{alg:single-linkage-cluster}
\end{algorithm}

\myparagraph{Analysis}

The initialization on Line \ref{alg:single-linkage-cluster:init} takes $\BigO{n}$ work and $\BigO{1}$ span. \citet{Jayanti21} proved that performing $m$ unionizations on a union-find data structure with $n$ elements takes $\BigO{m\left( \log(\frac{n}{m}+1) + \alpha(n) \right)}$ work, where $\alpha$ denotes the inverse Ackermann function. In our case, $m=n$. Therefore, the overall work complexity is $\BigO{n\alpha(n)}$. The unionization operation on Line \ref{alg:priority:unionize} takse span $\BigO{\log(n)}$. The overall span of the algorithm is therefore $\BigO{\log(n)}$.
\shangdi{This section can be combined with section 4 }

==> static-kd-tree.tex <==










 



















































